Language-Agnostic Suicidal Risk Detection Using Large Language Models

Suicidal risk detection in adolescents is a critical challenge, yet existing methods rely on language-specific models, limiting scalability and generalization. This study introduces a novel language-agnostic framework for suicidal risk assessment with large language models (LLMs). We generate Chinese transcripts from speech using an ASR model and then employ LLMs with prompt-based queries to extract suicidal risk-related features from these transcripts. The extracted features are retained in both Chinese and English to enable cross-linguistic analysis and then used to fine-tune corresponding pretrained language models independently. Experimental results show that our method achieves performance comparable to direct fine-tuning with ASR results or to models trained solely on Chinese suicidal risk-related features, demonstrating its potential to overcome language constraints and improve the robustness of suicidal risk assessment.

==> 2-RelatedWork.tex <==
\section{Related Works}
\subsection{Leveraging LLMs for Mental Health Detection}
The application of language models in mental health research domain has been expanding remarkably. For instance, Poswiata and Perelkiewicz~\cite{Poswiata2022OPILTEDIACL2022DS} introduced DepRoBERTa, a domain-specific variant of RoBERTa-large that was fine-tuned to detect depression states from social media text. With the advancement of LLMs, their use in mental health detection has gained increasing attention. Sadeghi et al.~\cite{Sadeghi2023ExploringTC} proposed an automated depression detection model by employing LLMs to extract depression-related features from the clinical interviews dataset. In a subsequent study~\cite{Sadeghi2024HarnessingMA}, they introduced a multimodal approach, integrating LLMs with facial expressions to predict depression severity. Similarly, Cui et al.~\cite{Cui2024SpontaneousSS} explored suicidal risk detection in adolescents using Whisper and LLMs by applying various fine-tuning strategies. Their approach incorporated automatic speech recognition (ASR) and evaluated different fusion techniques to integrate speech and text modalities, highlighting the potential of LLMs in suicidal risk assessment.


Employing LLMs has also supported a multilingual approach to mental health detection research. Skianis et al.~\cite{Skianis2024SeverityPI} addressed the lack of non-English mental health research by developing a multilingual adaptation of widely used mental health datasets. Besides, they translated English datasets into six languages to assess LLM's effectiveness in detecting mental health conditions across diverse linguistic contexts. Inspired by recent studies, we aim to develop a language-agnostic framework employing LLMs to extract multilingual suicidal risk-related features from transcriptions of Chinese speech data and subsequently compare their performance across language models of English and Chinese.
